Generic deformations of the colored sl(N)-homology for links

We generalize the works of Lee [arXiv:math/0210213v3] and Gornik [arXiv:math/0402266v2] to construct a basis for generic deformations of the colored sl(N)-homology defined in [arXiv:1002.2662v1]. As applications, we construct non-degenerate pairings and co-pairings which lead to dualities of generic deformations of the colored sl(N)-homology. We also define and study colored sl(N)-Rasmussen invariants. Among other things, we observe that these invariants vanish on amphicheiral knots and discuss some implications of this observation.

==> cross-+-slides.tex <==
\setlength{\unitlength}{1pt}
\begin{picture}(65,20)(-110,0)
\put(-100,-20){\vector(1,1){40}}

\put(-60,-20){\line(-1,1){15}}

\put(-85,5){\vector(-1,1){15}}

\put(-92,16){\tiny{$_m$}}

\put(-70,16){\tiny{$_n$}}

\put(-105,-20){\tiny{$\mathbb{A}$}}
\put(-105,15){\tiny{$\mathbb{X}$}}

\put(-55,-20){\tiny{$\mathbb{D}$}}
\put(-55,15){\tiny{$\mathbb{Y}$}}\end{picture}

==> cross---slides.tex <==
\setlength{\unitlength}{1pt}
\begin{picture}(65,20)(50,0)
\put(100,-20){\vector(-1,1){40}}

\put(60,-20){\line(1,1){15}}

\put(85,5){\vector(1,1){15}}

\put(68,16){\tiny{$_m$}}

\put(90,16){\tiny{$_n$}}

\put(55,-20){\tiny{$\mathbb{A}$}}
\put(55,15){\tiny{$\mathbb{X}$}}

\put(105,-20){\tiny{$\mathbb{D}$}}
\put(105,15){\tiny{$\mathbb{Y}$}}
\end{picture}

==> crossing-quasi-states-11+.tex <==
\setlength{\unitlength}{1pt}
\begin{picture}(40,40)(-20,-20)

\put(-20,-20){\vector(1,1){40}}

\put(20,-20){\line(-1,1){15}}

\put(-5,5){\vector(-1,1){15}}

\put(-11,15){\tiny{$_1$}}

\put(9,15){\tiny{$_1$}}

\put(-20,-10){\small{$a_1$}}

\put(-20,8){\small{$a_4$}}

\put(15,-10){\small{$a_2$}}

\put(15,8){\small{$a_3$}}

\put(-2,-15){$c$}

\end{picture}

==> crossing-quasi-states-11-.tex <==
\setlength{\unitlength}{1pt}
\begin{picture}(40,40)(-20,-20)

\put(20,-20){\vector(-1,1){40}}

\put(-20,-20){\line(1,1){15}}

\put(5,5){\vector(1,1){15}}

\put(-11,15){\tiny{$_1$}}

\put(9,15){\tiny{$_1$}}

\put(-20,-10){\small{$a_1$}}

\put(-20,8){\small{$a_4$}}

\put(15,-10){\small{$a_2$}}

\put(15,8){\small{$a_3$}}

\put(-2,-15){$c$}

\end{picture}

==> crossing-quasi-states-11-res0.tex <==
\setlength{\unitlength}{1pt}
\begin{picture}(80,55)(-40,-35)

\qbezier(-20,-20)(15,0)(-20,20)

\qbezier(20,-20)(-15,0)(20,20)

\put(-20,20){\vector(-2,1){0}}

\put(20,20){\vector(2,1){0}}

\put(-11,16){\tiny{$_1$}}

\put(9,16){\tiny{$_1$}}

\put(-40,0){\small{$a_1(=a_4)$}}


\put(10,0){\small{$a_2(=a_3)$}}

\put(-3,-35){$D^0$}

\end{picture}

==> decomp-IV-2-slide.tex <==
\setlength{\unitlength}{.75pt}
\begin{picture}(85,45)(-30,45)

\put(-20,0){\vector(0,1){45}}

\put(-20,45){\vector(0,1){45}}

\put(20,0){\vector(0,1){45}}

\put(20,45){\vector(0,1){45}}

\put(20,45){\vector(-1,0){40}}

\put(-27,20){\tiny{$_1$}}

\put(23,20){\tiny{$_{m+l-1}$}}

\put(-27,65){\tiny{$_l$}}

\put(23,65){\tiny{$_m$}}

\put(-5,38){\tiny{$_{l-1}$}}

\end{picture}

==> decomp-IV-3-slide.tex <==
\setlength{\unitlength}{.75pt}
\begin{picture}(65,45)(110,45)

\put(110,0){\vector(2,3){20}}

\put(150,0){\vector(-2,3){20}}

\put(130,30){\vector(0,1){30}}

\put(130,60){\vector(-2,3){20}}

\put(130,60){\vector(2,3){20}}

\put(117,20){\tiny{$_1$}}

\put(140,20){\tiny{$_{m+l-1}$}}

\put(117,65){\tiny{$_l$}}

\put(140,65){\tiny{$_m$}}

\put(133,42){\tiny{$_{m+l}$}}
\end{picture}

==> fork-sliding-general-10-slides.tex <==
\setlength{\unitlength}{1pt}
\begin{picture}(44,20)(-22,20)

\put(0,0){\line(0,1){8}}

\put(0,12){\vector(0,1){8}}

\put(0,20){\vector(1,1){20}}

\put(0,20){\vector(-1,1){20}}

\put(-20,10){\vector(1,0){40}}

\put(-13,35){\tiny{$_m$}}

\put(10,35){\tiny{$_l$}}

\put(3,2){\tiny{$_{m+l}$}}

\put(10,13){\tiny{$_n$}}

\end{picture}

==> fork-sliding-general-11-slides.tex <==
\setlength{\unitlength}{1pt}
\begin{picture}(44,20)(-22,20)

\put(0,0){\vector(0,1){20}}

\put(0,20){\line(1,1){8}}

\put(0,20){\line(-1,1){8}}

\put(12,32){\vector(1,1){8}}

\put(-12,32){\vector(-1,1){8}}

\put(-20,30){\vector(1,0){40}}

\put(-13,35){\tiny{$_m$}}

\put(10,35){\tiny{$_l$}}

\put(3,2){\tiny{$_{m+l}$}}

\put(12,26){\tiny{$_n$}}

\end{picture}

==> fork-sliding-general-12-slides.tex <==
\setlength{\unitlength}{1pt}
\begin{picture}(44,20)(-22,20)
\put(0,0){\vector(0,1){20}}

\put(0,20){\vector(1,1){20}}

\put(0,20){\vector(-1,1){20}}

\put(-20,10){\line(1,0){18}}

\put(2,10){\vector(1,0){18}}

\put(-13,35){\tiny{$_m$}}

\put(10,35){\tiny{$_l$}}

\put(3,2){\tiny{$_{m+l}$}}

\put(10,13){\tiny{$_n$}}

\end{picture}

==> fork-sliding-general-13-slides.tex <==
\setlength{\unitlength}{1pt}
\begin{picture}(44,20)(-22,20)
\put(0,0){\vector(0,1){20}}

\put(0,20){\vector(1,1){20}}

\put(0,20){\vector(-1,1){20}}

\put(-20,30){\line(1,0){8}}

\put(-8,30){\line(1,0){16}}

\put(12,30){\vector(1,0){8}}

\put(-13,35){\tiny{$_m$}}

\put(10,35){\tiny{$_l$}}

\put(3,2){\tiny{$_{m+l}$}}

\put(12,26){\tiny{$_n$}}

\end{picture}

==> fork-sliding-general-20-slides.tex <==
\setlength{\unitlength}{1pt}
\begin{picture}(44,20)(-22,20)

\put(0,0){\line(0,1){8}}

\put(0,12){\vector(0,1){8}}

\put(0,20){\vector(1,1){20}}

\put(0,20){\vector(-1,1){20}}

\put(20,10){\vector(-1,0){40}}

\put(-13,35){\tiny{$_m$}}

\put(10,35){\tiny{$_l$}}

\put(3,2){\tiny{$_{m+l}$}}

\put(10,13){\tiny{$_n$}}

\end{picture}

==> fork-sliding-general-21-slides.tex <==
\setlength{\unitlength}{1pt}
\begin{picture}(44,20)(-22,20)

\put(0,0){\vector(0,1){20}}

\put(0,20){\line(1,1){8}}

\put(0,20){\line(-1,1){8}}

\put(12,32){\vector(1,1){8}}

\put(-12,32){\vector(-1,1){8}}

\put(20,30){\vector(-1,0){40}}

\put(-13,35){\tiny{$_m$}}

\put(10,35){\tiny{$_l$}}

\put(3,2){\tiny{$_{m+l}$}}

\put(12,26){\tiny{$_n$}}

\end{picture}

==> fork-sliding-general-22-slides.tex <==
\setlength{\unitlength}{1pt}
\begin{picture}(44,20)(-22,20)

\put(0,0){\vector(0,1){20}}

\put(0,20){\vector(1,1){20}}

\put(0,20){\vector(-1,1){20}}

\put(20,10){\line(-1,0){18}}

\put(-2,10){\vector(-1,0){18}}

\put(-13,35){\tiny{$_m$}}

\put(10,35){\tiny{$_l$}}

\put(3,2){\tiny{$_{m+l}$}}

\put(10,13){\tiny{$_n$}}

\end{picture}

==> fork-sliding-general-23-slides.tex <==
\setlength{\unitlength}{1pt}
\begin{picture}(44,20)(-22,20)

\put(0,0){\vector(0,1){20}}

\put(0,20){\vector(1,1){20}}

\put(0,20){\vector(-1,1){20}}

\put(20,30){\line(-1,0){8}}

\put(8,30){\line(-1,0){16}}

\put(-12,30){\vector(-1,0){8}}

\put(-13,35){\tiny{$_m$}}

\put(10,35){\tiny{$_l$}}

\put(3,2){\tiny{$_{m+l}$}}

\put(12,26){\tiny{$_n$}}

\end{picture}

==> fork-sliding-general-30-slides.tex <==
\setlength{\unitlength}{1pt}
\begin{picture}(44,20)(-22,20)

\put(0,8){\vector(0,-1){8}}

\put(0,20){\line(0,-1){8}}

\put(20,40){\vector(-1,-1){20}}

\put(-20,40){\vector(1,-1){20}}

\put(-20,10){\vector(1,0){40}}

\put(-13,35){\tiny{$_m$}}

\put(10,35){\tiny{$_l$}}

\put(3,2){\tiny{$_{m+l}$}}

\put(10,13){\tiny{$_n$}}

\end{picture}

==> fork-sliding-general-31-slides.tex <==
\setlength{\unitlength}{1pt}
\begin{picture}(44,20)(-22,20)
\put(0,20){\vector(0,-1){20}}

\put(8,28){\vector(-1,-1){8}}

\put(-8,28){\vector(1,-1){8}}

\put(20,40){\line(-1,-1){8}}

\put(-20,40){\line(1,-1){8}}

\put(-20,30){\vector(1,0){40}}

\put(-14,36){\tiny{$_m$}}

\put(11,36){\tiny{$_l$}}

\put(3,2){\tiny{$_{m+l}$}}

\put(12,26){\tiny{$_n$}}

\end{picture}

==> fork-sliding-general-32-slides.tex <==
\setlength{\unitlength}{1pt}
\begin{picture}(44,20)(-22,20)

\put(0,20){\vector(0,-1){20}}

\put(20,40){\vector(-1,-1){20}}

\put(-20,40){\vector(1,-1){20}}

\put(-20,10){\line(1,0){18}}

\put(2,10){\vector(1,0){18}}

\put(-13,35){\tiny{$_m$}}

\put(10,35){\tiny{$_l$}}

\put(3,2){\tiny{$_{m+l}$}}

\put(10,13){\tiny{$_n$}}

\end{picture}

==> fork-sliding-general-33-slides.tex <==
\setlength{\unitlength}{1pt}
\begin{picture}(44,20)(-22,20)

\put(0,20){\vector(0,-1){20}}

\put(20,40){\vector(-1,-1){20}}

\put(-20,40){\vector(1,-1){20}}

\put(-20,30){\line(1,0){8}}

\put(-8,30){\line(1,0){16}}

\put(12,30){\vector(1,0){8}}

\put(-14,36){\tiny{$_m$}}

\put(11,36){\tiny{$_l$}}

\put(3,2){\tiny{$_{m+l}$}}

\put(12,26){\tiny{$_n$}}

\end{picture}

==> fork-sliding-general-40-slides.tex <==
\setlength{\unitlength}{1pt}
\begin{picture}(44,20)(-22,20)

\put(0,8){\vector(0,-1){8}}

\put(0,20){\line(0,-1){8}}

\put(20,40){\vector(-1,-1){20}}

\put(-20,40){\vector(1,-1){20}}

\put(20,10){\vector(-1,0){40}}

\put(-13,35){\tiny{$_m$}}

\put(10,35){\tiny{$_l$}}

\put(3,2){\tiny{$_{m+l}$}}

\put(10,13){\tiny{$_n$}}

\end{picture}

==> fork-sliding-general-41-slides.tex <==
\setlength{\unitlength}{1pt}
\begin{picture}(44,20)(-22,20)

\put(0,20){\vector(0,-1){20}}

\put(8,28){\vector(-1,-1){8}}

\put(-8,28){\vector(1,-1){8}}

\put(20,40){\line(-1,-1){8}}

\put(-20,40){\line(1,-1){8}}

\put(20,30){\vector(-1,0){40}}

\put(-14,36){\tiny{$_m$}}

\put(11,36){\tiny{$_l$}}

\put(3,2){\tiny{$_{m+l}$}}

\put(12,26){\tiny{$_n$}}

\end{picture}

==> fork-sliding-general-42-slides.tex <==
\setlength{\unitlength}{1pt}
\begin{picture}(44,20)(-22,20)

\put(0,20){\vector(0,-1){20}}

\put(20,40){\vector(-1,-1){20}}

\put(-20,40){\vector(1,-1){20}}

\put(20,10){\line(-1,0){18}}

\put(-2,10){\vector(-1,0){18}}

\put(-13,35){\tiny{$_m$}}

\put(10,35){\tiny{$_l$}}

\put(3,2){\tiny{$_{m+l}$}}

\put(10,13){\tiny{$_n$}}

\end{picture}

==> fork-sliding-general-43-slides.tex <==
\setlength{\unitlength}{1pt}
\begin{picture}(44,20)(-22,20)

\put(0,20){\vector(0,-1){20}}

\put(20,40){\vector(-1,-1){20}}

\put(-20,40){\vector(1,-1){20}}

\put(20,30){\line(-1,0){8}}

\put(8,30){\line(-1,0){16}}

\put(-12,30){\vector(-1,0){8}}

\put(-14,36){\tiny{$_m$}}

\put(11,36){\tiny{$_l$}}

\put(3,2){\tiny{$_{m+l}$}}

\put(12,26){\tiny{$_n$}}

\end{picture}

==> v-vector-m+n-slide.tex <==
\setlength{\unitlength}{.5pt}
\begin{picture}(40,40)(-20,40)
\put(0,0){\vector(0,1){80}}
\put(5,75){\tiny{$_{m+n}$}}
\end{picture}
